The Fine-Grained and Parallel Complexity of Andersen's Pointer Analysis

Pointer analysis is one of the fundamental problems in static program analysis. Given a set of pointers, the task is to produce a useful over-approximation of the memory locations that each pointer may point-to at runtime. The most common formulation is Andersen's Pointer Analysis (APA), defined as an inclusion-based set of $m$ pointer constraints over a set of $n$ pointers. Existing algorithms solve APA in $O(n^2\cdot m)$ time, while it has been conjectured that the problem has no truly sub-cubic algorithm, with a proof so far having remained elusive. In this work we draw a rich fine-grained and parallel complexity landscape of APA, and present upper and lower bounds. First, we establish an $O(n^3)$ upper-bound for general APA, improving over $O(n^2\cdot m)$ as $n=O(m)$. Second, we show that even on-demand APA ("may a specific pointer $a$ point to a specific location $b$?") has an $\Omega(n^3)$ (combinatorial) lower bound under standard complexity-theoretic hypotheses. This formally establishes the long-conjectured "cubic bottleneck" of APA, and shows that our $O(n^3)$-time algorithm is optimal. Third, we show that under mild restrictions, APA is solvable in $\tilde{O}(n^{\omega})$ time, where $\omega<2.373$ is the matrix-multiplication exponent. It is believed that $\omega=2+o(1)$, in which case this bound becomes quadratic. Fourth, we show that even under such restrictions, even the on-demand problem has an $\Omega(n^2)$ lower bound under standard complexity-theoretic hypotheses, and hence our algorithm is optimal when $\omega=2+o(1)$. Fifth, we study the parallelizability of APA and establish lower and upper bounds: (i) in general, the problem is P-complete and hence unlikely parallelizable, whereas (ii) under mild restrictions, the problem is parallelizable. Our theoretical treatment formalizes several insights that can lead to practical improvements in the future.

==> algorithms/algo_cubic_bk.tex <==
\smallskip
\begin{algorithm}%[H]
\small
\DontPrintSemicolon
\SetInd{0.3em}{0.3em}
\caption{$\AlgoCubic$}\label{algo:cubic}
\SetKwFunction{ProcessEps}{$\ProcessEpsilon$}
%\SetKwFunction{ProcessRef}{$\ProcessRef$}
\SetKwProg{Fn}{Function}{:}{}
\KwIn{
An instance $(A,S)$ of $\APA$.
}
\KwOut{A set $(a,b)$ of all points-to relationships $b\in \PointsToSet{a}$.}
\BlankLine
\begin{multicols}{3}
\tcp{Initialization}
Let $\Worklist, \Done\gets \emptyset$\\
\ForEach{$a=\&b$}{\label{line_cubic_init1}
Insert $(b,a,\&)$ in $\Worklist$\\
Insert $(b,a,\&)$ in $\Done$
}
\ForEach{$a=b$}{\label{line_cubic_init2}
Insert $(b,a,\epsilon)$ in $\Worklist$\\
Insert $(b,a,\epsilon)$ in $\Done$
}
\tcp{Computation}
\While{$\Worklist\neq \emptyset$}{\label{line:cubic_main_loop}
Extract $(a,b,t)$ from $\Worklist$\\
\eIf{$t=\epsilon$}{
$\ProcessEpsilon(a,b)$
}
{
$\ProcessRef(a,b)$
}
}
\Return{$\{(a,b)\colon (b,a,\&) \in \Done \}$}
\pagebreak
%\vspace{5em}

\tcp{Process inclusion edges}
\Fn{\ProcessEps{$a$, $b$}}{
\ForEach{$(b,c,\epsilon)\in \Done$}{\label{line:proceps1}
$\Establish(a,c,\epsilon)$
%\uIf{$a\DEdge{\epsilon}c$ is not in $\Done$}{
%Insert $a\DEdge{\epsilon}c$ in $\Worklist$\\
%Insert $a\DEdge{\epsilon}c$ in $\Done$\\
%}
}
\ForEach{$(c,a,\epsilon)\in \Done$}{\label{line:proceps2}
$\Establish(c,b,\epsilon)$
%\uIf{$c\DEdge{\epsilon}b$ is not in $\Done$}{
%Insert $c\DEdge{\epsilon}b$ in $\Worklist$\\
%Insert $c\DEdge{\epsilon}b$ in $\Done$\\
%}
}
\ForEach{$(c,a,\&)\in\Done$}{\label{line:proceps3}
$\Establish(c,b,\&)$
%\uIf{$c\DEdge{\&}b$ is not in $\Done$}{
%Insert $c\DEdge{\&}b$ in $\Worklist$\\
%Insert $c\DEdge{\&}b$ in $\Done$\\
%}
}
}

\BlankLine
\BlankLine
\BlankLine
\tcp{Establish new inclusion and reference edges}
\SetKwFunction{ProcessEstablish}{$\Establish$}
\Fn{\ProcessEstablish{$a,b,t$}}{
\uIf{$(a,c,t)\not \in\Done$}{
Insert $(a,c,t)$ in $\Worklist$\\
Insert $(a,c,t)$ in $\Done$\\
}
}

\pagebreak
\tcp{Process reference edges}
\SetKwFunction{ProcessEps}{$\ProcessRef$}
\Fn{\ProcessEps{$a$, $b$}}{
\ForEach{$(b,c,\epsilon)\in\Done$}{\label{line:procref1}
$\Establish(a, c, \&)$
%\uIf{$a\DEdge{\&}c$ is not in $\Done$}{
%Insert $a\DEdge{\&}c$ in $\Worklist$\\
%Insert $a\DEdge{\&}c$ in $\Done$\\
%}
}
\ForEach{$c=*b$ in $S$}{\label{line:procref2}
$\Establish(a, c, \epsilon)$
%\uIf{$a\DEdge{\epsilon}c$ is not in $\Done$}{
%Insert $a\DEdge{\epsilon}c$ in $\Worklist$\\
%Insert $a\DEdge{\epsilon}c$ in $\Done$\\
%}
}
\ForEach{$*b=c$ in $S$}{\label{line:procref3}
$\Establish(c, a, \epsilon)$
%\uIf{$c\DEdge{\epsilon}a$ is not in $\Done$}{
%Insert $c\DEdge{\epsilon}a$ in $\Worklist$\\
%Insert $c\DEdge{\epsilon}a$ in $\Done$\\
%}
}
}
\end{multicols}
\end{algorithm}





==> algorithms/algo_diff_prop_stack.tex <==
\smallskip
\begin{algorithm}%[H]
\small
\DontPrintSemicolon
\SetInd{0.3em}{0.3em}
\caption{$\AlgoDiffPropStack$}\label{algo:diff_prop_stack}
\SetKwFunction{ProcessEps}{$\ProcessEpsilon$}
%\SetKwFunction{ProcessRef}{$\ProcessRef$}
\SetKwProg{Fn}{Function}{:}{}
\KwIn{
An instance $(A,S)$ of $\APA$.
}
\KwOut{A set $(a,b)$ of all points-to relationships $b\in \PointsToSet{a}$.}
\BlankLine
\begin{multicols}{3}
\tcp{Initialization}
Initialize a map of stacks $\PointsToStack\colon A\to A^*$\\
Initialize a worklist $\Worklist$\\
\ForEach{statement $\mathsf{i\colon x = new T()}$}{
Push $o_i$ in $\PointsToStack[x]$\\
Add $x$ to $\Worklist$\\
}
\ForEach{statement $\mathsf{x=y}$}{
Add edge $y\to x$ in $G$.
}

\pagebreak
\tcp{Computation}
\While{$\Worklist$ is not empty}{
Extract $n$ from $\Worklist$\\

}
\end{multicols}
\end{algorithm}





==> algorithms/algo_diff_prop_stack_bk.tex <==
\smallskip
\begin{algorithm}%[H]
\small
\DontPrintSemicolon
\SetInd{0.3em}{0.3em}
\caption{$\AlgoDiffPropStack$}\label{algo:diff_prop_stack}
\SetKwFunction{ProcessEps}{$\ProcessEpsilon$}
%\SetKwFunction{ProcessRef}{$\ProcessRef$}
\SetKwProg{Fn}{Function}{:}{}
\KwIn{
An instance $(A,S)$ of $\APA$.
}
\KwOut{A set $(a,b)$ of all points-to relationships $b\in \PointsToSet{a}$.}
\BlankLine
\begin{multicols}{3}
\tcp{Initialization}
Initialize a map of stacks $\PointsToStack\colon A\to A^*$\\
Initialize a worklist $\Worklist$\\
\ForEach{statement $\mathsf{i\colon x = new T()}$}{
Push $o_i$ in $\PointsToStack[x]$\\
Add $x$ to $\Worklist$\\
}
\ForEach{statement $\mathsf{x=y}$}{
Add edge $y\to x$ in $G$.
}

\pagebreak
\tcp{Computation}
\While{$\Worklist$ is not empty}{
Extract $n$ from $\Worklist$\\

}
\end{multicols}
\end{algorithm}





==> dyckreduction.tex <==
\section{Reduction to Dyck Reachability}\label{sec:dyckreduction}


\input{figures/fig_dyck_reduction}
%\input{figure/fig_dyck_reduction2}

==> experiments.tex <==
\section{Experiments}\label{sec:experiments}

==> linear.tex <==
\subsection{Sparse Andersen's Pointer Analysis in $O(n^{3/2})$ Time}\label{subsec:linear}

We now turn our attention to sparse instances of $\APA$.
This is a relevant setting as natural conventions in some programming languages yield sparse instances.
The sparsity conditions are stated on the underlying final flow graph, see~\cite{Sridharan09} for details.
Under the sparsity conditions, that work decreases the $\APA$ analysis time to $O(n^2)$.
Here we show that sparsity on the final Dyck graph allows reducing this bound to $O(n^{3/2})$.
We start by making the sparsity conditions precise.

\Paragraph{Sparse final Dyck graphs.}
We now define in detail the flow graph, which is the standard data-structure used in the literature to perform $\APA$.
Consider \cref{algo:cubic} from the previous section, and let $\hat{G}=(A, \hat{E})$ be the Dyck graph by taking the edge set $\hat{E}$ to be the set $\Done$ after termination of the algorithm.
Following \cite{Sridharan09}, given a constant $c>0$, the instance $(A,S)$ is \emph{$c$-sparse}
if the following conditions hold.
\begin{compactenum}
\item $|\hat{E}|\leq c\cdot n$.
\item For every pointer $a$, there are at most $c$ statements of type~3 and type~4 that dereference $a$.
\item Every pointer $a$ is referenced at most $c$ times\footnote{Although this condition is not made explicit in~\cite{Sridharan09}, it is directly implied by the condition that each program method has constant size. See \cite[Section 4.2]{Sridharan09} for details.}.
\end{compactenum}
We let $\SparseAPAPA$ be the $\APAPA$ problem restricted to $c$-sparse inputs, for some constant $c$.
We show that our previous algorithm $\AlgoCubic$ (\cref{algo:cubic}) yields an $O(n^{3/2})$ time bound for $\SparseAPAPA$.


\Paragraph{Complexity analysis.}
We first set up some helpful notation.
Given a pointer $a$, we let
\begin{align*}
%p_a=|\{ b\in A\colon (b,a)\in \hat{E} \}| \cdot |\{ b\in A\colon (a,b)\in \hat{E} \}| \qquad \text{and} \qquad 
q_a=|c\in A\colon (c,a,\&)\in \hat{E}| \cdot |\{ b\in A\colon (a,b, \epsilon)\in \hat{E} \}|\ ,
\end{align*}
%i.e., $p_a$ is the product of the incoming and outgoing neighbors of $a$ in the flow graph $\hat{G}$,
i.e., $q_a$ is the product of the size of the points-to set of $a$ with the outgoing neighbors of $a$ in $\hat{G}$.
Our complexity analysis relies on the following key insights.
\begin{compactenum}
\item In general, there exist pointers with points-to sets that have size linear in $n$.
At a first glance, this results in a quadratic bound in the total size of all points-to sets.
%Indeed, this is also stated in~\cite{Sridharan09}.
However, a tighter analysis shows that, despite some large points-to sets, the average size of points-to sets is only constant.
\item Assume that an inclusion edge $(a,b, \epsilon)$ has just been extracted from the worklist in \cref{line:cubic_main_loop}, and consider the loop in \cref{line:proceps3}.
As the algorithm performs a form of transitive closure, it will iterate over all nodes $c$ for which it is already established that $(c,a,\&)$,
and will establish that $(c,b,\&)$ also holds by transitivity.
At a first glance, this results in a quadratic bound, as by sparsity there are $O(n)$ edges $(c,a,\&)$, and for each such edge there are $O(n)$ pointers $b$ for which we might discover that $(a,b,\epsilon)$.
Note, however, that this counting argument overshoots, as it will result in $\Theta(n^2)$ edges $(c,b,\&)$, which violates the sparsity of $(A,S)$.
A tighter observation is that for every pointer $b$, the loop will be executed $q_a$ times.
In addition, $q_a$ counts (asymptotically) the number of triangles of $\hat{G}$ that contain $a$.
Summing over all $a$, the number of times that the loop is executed is bounded by the number of triangles in $\hat{G}$, which is only $O(n^{3/2})$~\cite{Suri11}.
\end{compactenum}



The above intuition is formally captured in the following lemma.

\smallskip
\begin{restatable}{lemma}{lemsparseptsize}\label{lem:sparse_pt_size}
We have
(i)~$\sum_{a\in A} |\PointsToSet{a}| = O(n)$ and (ii)~$\sum_{a\in A} q_a = O(n^{3/2})$.
\end{restatable}

Based on \cref{lem:sparse_pt_size} we prove \cref{them:sparse_faster}.

\begin{proof}[Proof of \cref{them:sparse_faster}]
%The correctness of $\AlgoCubic$ is argued in \cref{them:cubic_upper_bound}, so here we argue about the improved complexity on sparse inputs.
We first consider the initialization phase.
The first loop in \cref{line_cubic_init1} is executed $O(n)$ times, since by sparsity, every pointer is referenced at most $c=O(1)$ times.
The second loop in \cref{line_cubic_init2} is executed $O(n)$ times, since every iteration results in an edge in the flow graph $\hat{G}$, and we have $|\hat{E}|=O(n)$, by sparsity.

We now proceed to the function $\ProcessEpsilon$.
%It is straightforward to see that, for a fixed pointer $b$, the loop in \cref{line:proceps1} is executed at most $p_b$ times.
%Similarly, for a fixed pointer $a$, the loop in \cref{line:proceps2} is executed at most $p_a$ times, 
It is straightforward to see that, for a fixed pointer $a$, the loop in \cref{line:proceps3} is executed at most $q_a$ times.
By \cref{lem:sparse_pt_size}, we have $\sum_{a\in A} q_a=O(n^{3/2})$, hence the total running time for the function $\ProcessEpsilon$ is $O(n^{3/2})$.

We proceed to the function $\ProcessRef$.
Similarly as before, for a fixed pointer $b$, the loop in \cref{line:procref1} is executed at most $q_b$ times, and thus the loop takes $O(n^{3/2})$ total time for all pointers.
Now we turn our attention to the loops in \cref{line:procref2} and \cref{line:procref3}.
Given a pointer $b$, let $r_b$ be an upper-bound on number of statements of type~3  and type~4 that dererference $b$.
By sparsity, we have $r_b\leq c=O(1)$. 
The number of times that each of the loops in \cref{line:procref2} and \cref{line:procref3} is executed is bounded by
\begin{align*}
\sum_{b\in A} |\PointsToSet{b}| \cdot r_b\leq c\cdot \sum_{b\in A} |\PointsToSet{b}| = c\cdot O(n) = O(n)\ ,
\end{align*}
where the second-to-last equality follows from point (i) of \cref{lem:sparse_pt_size}.
Hence the total running time for the function $\ProcessRef$ is $O(n^{3/2}) + O(n)=O(n^{3/2})$.

Finally, note that in our analysis, we have used constant time for the operations of set insertion and membership.
This can be easily achieved by implementing each set as a bit-array. 
Since some of the sets can be of size  $\Theta(n)$ (e.g., for storing the neighbors of a high-degree node),
performing a naive initialization to all sets would require $\Theta(n^2)$ time.
We avoid this cost by using a known technique for constant-time array initialization, regardless of the size of the set~\cite{Aho74}.
Hence the total time for initializing the data structures is $O(n)$.

The desired result follows.
\end{proof}



==> problems.tex <==
\subsection{Computational Problems}\label{subsec:problems}

\Paragraph{Andersen Pointer Analysis.}

\Paragraph{Bounded Andersen Pointer Analysis.}

\Paragraph{Dyck Reachability.}

==> proof_cubic.tex <==
\subsection{Proofs of \cref{sec:cubic}}\label{appsubsec:proof_cubic}

\smallskip
\lemsparseptsize*
\begin{proof}
Consider the flow graph $\hat{G}=(A,\hat{E})$.
Given a pointer $a\in A$, let $n_a=\{ b\in A\colon a=\&b \}$, i.e., $n_a$ is the number of pointers referenced by $a$ in the input.

For (i), by the sparsity of the input, we have $n_a\leq c$ for each $a\in A$.
Thus,
\begin{align*}
\sum_{a\in A} \PointsToSet{a} = \sum_{a\in A} \left(n_a + \sum_{b\colon (b,a)\in \hat{E}} n_b\right)\leq \sum_{a\in A} c + \sum_{(b,a)\in \hat{E}} c \leq |A|\cdot c + |\hat{E}| \cdot c\leq  n\cdot c + n\cdot c^2 = O(n)\ .
\end{align*}

For (ii) and (iii), we argue as follows.
Consider a Dyck graph $H=(A,R)$, where
\begin{align*}
R=\{ (a,b,\epsilon)\colon (a,b)\in \hat{E} \} \cup \{ (a,b,\&)\colon a\in \PointsToSet{b} \}
\end{align*}
and note that
\begin{align*}
|R|=|\hat{E}| + \sum_{a\in A} |\PointsToSet{a}| \leq c\cdot n \cdot O(n) = O(n)\ ,
\end{align*}
as by (i)~, we have $\sum_{a\in A} |\PointsToSet{a}|=O(n)$.

Since $\hat{G}$ is transitively closed, for every triplet of pointers $(a,b,c)$ such that $(b,a), (a,c)\in \hat{E}$, we have $(b,c)\in \hat{E}$.
Hence the sum $\sum_{a\in A} p_a$ is bounded by the number of triangles in $H$ (in particular, the ones formed by $\epsilon$-labeled edges).
Similarly, by the definition of points-to sets, for every triplet of pointers $(a,b,c)$ such that $a\in \PointsToSet{b}$ and $(b,c)\in \hat{E}$, we have $a\in \PointsToSet{c}$.
Hence, the sum $\sum_{a\in A} q_a$ is bounded by the number of triangles in $H$ (in particular, the ones formed by two $\&$-labeled edges and one $\epsilon$-labeled edge).

It is known that the number of triangles in a graph with $k$ edges is $O(k^{3/2})$~\cite{Suri11}.
Hence the number of triangles in $H$ is bounded by $O(|R|^{3/2})=O(n^{3/2})$.

The desired result follows.
\end{proof}


==> related_work.tex <==
\subsection{Other Related Work}\label{subsec:related_work}
